Resisting Manipulative Bots in Meme Coin Copy Trading: A Multi-Agent Approach with Chain-of-Thought Reasoning

Copy trading has become the dominant entry strategy in meme coin markets. However, due to the market's extremely illiquid and volatile nature, the strategy exposes an exploitable attack surface: adversaries deploy manipulative bots to front-run trades, conceal positions, and fabricate sentiment, systematically extracting value from na\"ive copiers at scale. Despite its prevalence, bot-driven manipulation remains largely unexplored, and no robust defensive framework exists. We propose a manipulation-resistant copy-trading system based on a multi-agent architecture powered by a multi-modal large language model (LLM) and chain-of-thought (CoT) reasoning. Our approach outperforms zero-shot and most statistic-driven baselines in prediction accuracy as well as all baselines in economic performance, achieving an average copier return of 3% per meme coin investment under realistic market frictions. Overall, our results demonstrate the effectiveness of agent-based defenses and predictability of trader profitability in adversarial meme coin markets, providing a practical foundation for robust copy trading.

==> Equations/sol_concavity.tex <==
\begin{equation}
    \small
    \label{eq:sol_concavity}
    y = y' - \frac{k}{x + x'}.
\end{equation}

==> Exhibits/bot.tex <==
\begin{figure}[b]
\centering
\begin{minipage}[t]{0.53\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/copytrade.png}
    \caption{GMGN Copy Trading.}
    \label{fig:copytrade}
\end{minipage}
\hfill
\begin{minipage}[t]{0.46\linewidth}
    \centering
    \includegraphics[width=0.96\linewidth]{Figures/bot.png}
    \caption{A Telegram Bot.}
    \label{fig:bot_as_a_service}
\end{minipage}
\end{figure}


==> Exhibits/candle.tex <==
\begin{figure}[tb]
  \centering
  \begin{subfigure}{0.49\linewidth}
      \centering
        \includegraphics[width=\linewidth]{Figures/candle_good.png}
      \caption{Meme coin project with good farming opportunity.}
      \label{subfig:candle_good}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.49\linewidth}
      \centering
      \includegraphics[width=\linewidth]{Figures/candle_poor.png}
      \caption{Meme coin project with poor farming opportunity.}
      \label{subfig:candle_poor}
    \end{subfigure}
  \caption{Pre-migration candlestick chart.}
  \label{fig:bonding_curve}
\end{figure}

==> Exhibits/case.tex <==
\begin{figure*}[tb]
    \centering
    \includegraphics[width=\linewidth]{Figures/case.pdf}
    \caption{The impact of manipulative bots on the life cycle of a meme coin: a case study of MAO. A timeline highlights key events, which are mapped to the corresponding candlestick segments (framed by color boxes). These candlesticks are then linked to the underlying on-chain transaction and comment histories.}
    \label{fig:case}
\end{figure*}

==> Exhibits/forest_plot.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{Figures/forest_plot_mdd.pdf}
    \caption{Coefficient of Single-factor Model.}
    \label{fig:forest_plot_mdd}
\end{figure}

==> Exhibits/gmgn.tex <==
\begin{figure}[tb]
  \centering
  \begin{subfigure}{\linewidth}
      \centering
        \includegraphics[width=\linewidth]{Figures/gmgn_copytrading.png}
      \caption{GMGN KOL dashboard.}
      \label{subfig:gmgn_copytrading}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
      \centering
      \includegraphics[width=\linewidth]{Figures/gmgn_kol.png}
      \caption{GMGN Copytrading}
      \label{subfig:gmgn_kol}
    \end{subfigure}
  \caption{Memecoin-trading website.}
  \label{fig:gmgn}
\end{figure}

==> Exhibits/historical_meme.tex <==
\begin{figure}[tb]
\centering
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/historical_meme_pool.pdf}
  \caption{Number of Uniswap V3 or Raydium Pools.}
  \label{subfig:historical_meme_pool}
\end{subfigure}
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/historical_meme_token.pdf}
  \caption{Number of Uniswap V3 or Raydium Tokens.}
  \label{subfig:historical_meme_token}
\end{subfigure}
\caption{.}
\label{fig:historical_meme}
\end{figure}

==> Exhibits/mdd_survival.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{Figures/mdd_survival.pdf}
    \caption{Survival Analysis.}
    \label{fig:mdd_survival}
\end{figure}

==> Exhibits/pnut.tex <==
\begin{figure}[tb]
  \centering
  % \begin{subfigure}{\linewidth}
  %     \centering
  %     \includegraphics[width=0.75\linewidth]{Figures/pnut.png}
  %     \caption{Peanut the Squirrel, one of the most well-known meme coins launched on Pump.fun, reached a market capitalization of \$69,000 after 800 million coins were purchased, fully completing its bonding curve. Subsequently, 200 million Peanut the Squirrel coins were migrated to the \ac{dex}.}
  %     \label{subfig:pnut}
  %   \end{subfigure}
  %   \vfill
    % \begin{subfigure}{\linewidth}
      \centering
      \includegraphics[width=\linewidth]{Figures/bonding_curve.pdf}
      % \caption{Red solid line describes the relationship between the total SOL deposited by traders and the total meme coins received. From this, the price of the meme coin in terms of SOL can also be derived (blue solid line). Blue and red dotted lines are the initial price and migration price. $x'$ and $y'$ are 30 and 1,073,000,191, respectively}
      \label{subfig:bonding_curve}
    % \end{subfigure}

  \caption{Bonding curve mechanism. Red solid line describes the relationship between the total SOL deposited by traders and the total meme coins received. From this, the price of the meme coin in terms of SOL can also be derived (blue solid line). Blue and red dotted lines are the initial price and migration price. $x'$ and $y'$ are 30 and 1,073,000,191, respectively}
  \label{fig:bonding_curve}
\end{figure}

==> Exhibits/profit.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{Figures/profit_cs.pdf}
    \caption{Cumulative profit of \ac{kol} wallets of the meme coins with strong farming opportunity.}
    \label{fig:profit}
\end{figure}

==> Exhibits/ret.tex <==
\begin{figure}[tb]
\centering
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/ret_1h_all.pdf}
  \caption{.}
  \label{subfig:ret_1h_all}
\end{subfigure}%
\hfill
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/ret_1h_greater_-0.5.pdf}
  \caption{.}
  \label{subfig:ret_1h_greater_-0.5}
\end{subfigure}%
\hfill
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/ret_1h_lower_-0.5.pdf}
  \caption{.}
  \label{subfig:ret_1h_lower_-0.5}
\end{subfigure}
\caption{.}
\label{fig:ret}
\end{figure}

==> Exhibits/ridge.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{Figures/ridge.pdf}
    \caption{Profit distributions for a \acs{kol}/bump bot/sniper bot (\href{https://solscan.io/account/CcSVw6PGY655z9ava7pQhSkckmBL7rtkrjPGRVK5z1K3}{CcS..1K3}), a noise trader (\href{https://solscan.io/account/E9D2wrgjfhbaopWjgkiwX4o9eVFjLQhUiCr5SBiZMpWn}{E9D..pWn}), and an underperforming trader/bump bot (\href{https://solscan.io/account/J8JSA7BGKmauruAD8A7fWwwz9UoPvbEKPksW1WDsqcd1}{J8J..cd1}). The dashed line indicates the mean profit across all memecoin projects in which each trader participated. The light shading shows the Gaussian kernel density estimates of project-level trading profits, while the darker shading marks the 99\% $t$-confidence interval for the mean profit of each trader.}
    \label{fig:ridge}
\end{figure}

==> Exhibits/token_creation.tex <==
\begin{figure*}[tb]
  \centering
      \includegraphics[width=\linewidth]{Figures/token_creation.png}
  \caption{\textbf{Meme Coin Creation Illustration}\\Users can upload an image and select a name and ticker. Pumpfun will use this information to create a new meme coin.}
  \label{fig:token_creation}
\end{figure*}

==> Exhibits/trading_page.tex <==
\begin{figure*}[H]
  \centering
      \includegraphics[width=\linewidth]{Figures/trading_page.png}
  \caption{Pumpfun Trading Page. Pump.fun marks transaction bundles, groups of transactions occurring within the same block, as possible bot activity. On the right-hand side, it also displays token holders and their corresponding holdings.}
  \label{fig:tradingpage}
\end{figure*}

==> Exhibits/txn_dis.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/txn_dis.pdf}
    \caption{Distribution of token transactions in 12 hours.}
    \label{fig:txn_dis}
\end{figure}

==> Exhibits/wallet.tex <==
\begin{table}[tb]
    \centering
    \small
    \caption{Performance of the wallet evaluation agent using \ac{cot} prompting. “TRUE” indicates that the wallet achieved a positive profit while trading a specific meme coin and qualified as a KOL, whereas “FALSE” indicates otherwise.}
    \input{Tables/wallet}   
    \label{tab:wallet}
\end{table}

==> Exhibits/webpage.tex <==
\begin{figure*}[H]
  \centering
      \includegraphics[width=\linewidth]{Figures/webpage.png}
  \caption{Pumpfun Frontpage Meme Coin Bumping. Each time a transaction occurs for a meme coin, it gets bumped to the front page and briefly jiggles, increasing its visibility and exposure.}
  \label{fig:webpage}
\end{figure*}

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> Prompt/w_cot.tex <==
% \begin{reasoning}[label={cot:w_cot}]{Exemplar.}

% \includegraphics[width=\linewidth]{Figures/candle_bad_gradual.png}

% \begin{lstlisting}[
%   style=jsonplain,
%   caption={Schema-based Reasoning (Positive Case)},
% ]
% {"reasoning":{"Statistical Significance":"Gate check: require t-statistic > 1.645 (one-tailed 5%). Observed = 24.39. Since 24.39 > 1.645, the gate passes.","Activity and Longevity":"Recency requires time since last trade < 86400s: 371 < 86400 passes. Longevity prefers time since first trade > 31536000s: 19118974 < 31536000 not met. Longevity is a preference, not a veto.","Summary":"All core checks pass (significance, profitability, risk control, temporal robustness, and sample size). Despite not meeting the one-year longevity preference, the wallet remains attractive for next-trade copy trading."},"result":true}
% \end{lstlisting}
% \end{reasoning}

\begin{reasoning}[label={cot:w_cot}]{Exemplar.}

\begin{minipage}[t]{0.48\linewidth}
\includegraphics[width=\linewidth]{Figures/candle_bad_gradual_1.png}
\end{minipage}\hfill
\begin{minipage}[t]{0.48\linewidth}

\begin{lstlisting}[
  style=jsonplain,
  caption={Schema-based Reasoning (Positive Case)},
]
...
\end{lstlisting}

\end{minipage}

\end{reasoning}

==> Sections/case.tex <==
\section{A Meme Coin Case Study}
\input{Exhibits/case}

To investigate how manipulative bots influence the lifecycle of a meme coin, we present a case study in \autoref{fig:case}. We select \href{https://pump.fun/coin/2F84uaBysP4sD7Qby33fAM9RrSzhcR9KWrUT1ixwpump}{MAO} as a presentative example because it exhibits all four types of bots discussed in \autoref{subsec:bot}. While not all meme coins feature every type of bot, this case illustrates their mechanisms and clarifies how bots shape the lifecycle of a meme coin. For simplicity, wallet addresses are abbreviated to their first five characters.

\subsection{Token Creation and Launch Bundle}
At 15:06:24 on January 17, 2025, in block 314596960, token creator wallet 7xA7A created meme coin MAO, marked as stage 1 on the timeline in \autoref{fig:case}. Within the same block, the creator employs an automated script to generate multiple fresh wallets (e.g., 712nX, 6fYzn, and 4hZpo) and purchase MAO, as shown by the red box in the left-hand transaction history panel in \autoref{fig:case}. This behavior exemplifies the launch bundle described in \autoref{subsubsec:bundle}, whereby newly created wallets fabricate trading activity, artificially inflate the coin price, and conceal the creator's true position.

\subsection{Sniper Bot Front-Running}
Only four blocks and one second after the launch, the sniper wallet EW6Dk front-ran all other retail traders and purchased the meme coin (orange box and stage 2). This automated sniper bot secured a relatively low entry price through its speed advantage while slightly inflating the coin's price.

\subsection{Comment and Bump Bot}
From 15:10:17 to 16:26:42, comment bots disseminated fabricated positive messages (blue box and stage 3), such as \enquote{SENDOOR}, a term suggesting that the meme coin would accumulate sufficient market capitalization to migrate. This behavior created the illusion of active community communication and lured uninformed traders to participate. Between 15:37:36 and 16:40:45, the bump bot 4h7Lk.. repeatedly bought and sold the same amount of MAO (purple box and stage 4). Each transaction was bumped to the front page of Pumpfun, thereby attracting additional users.

\subsection{Rug Pull}
At 16:40:54, the creator and associated launch bundles began selling their holdings with a significant profit, causing the meme coin’s price to drop sharply within a minute (red box and stage 5). The sniper then detected this movement and exited its position with a moderate profit (orange box and stage 5). Ultimately, most retail traders closed their holdings with a loss. 

We also visualize the two key performance metrics for meme coin projects: \begin{enumerate*}\item The vertical dashed gray line indicates the maximum return, defined as the return between the initial price and the peak price. \item The horizontal dashed gray line denotes dump duration, measured as the time in seconds from the peak time to the point where the price falls to 10\% of its peak price.\end{enumerate*} 

==> Tables/feature_importance.tex <==
\begin{tabularx}{0.82\linewidth}{l*{3}{X}}
\toprule
\multirow{2}{*}{\textbf{\makecell{Feature}}} & \multicolumn{3}{c}{\textbf{Normalized Importance}} \\
\cmidrule(lr){2-4}
 & \makecell{LASSO} & \makecell{NN} & \makecell{XGBoost} \\
\midrule
Trader Purchase Amount & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.2214}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.1684}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.1320}} \\
$t$-stat & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.1833}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.1491}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.1127}} \\
Return (6th--10th) & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0684}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0790}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.1045}} \\
Return (1st--5th) & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0495}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0777}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.1017}} \\
Return Standard Deviation & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0689}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0509}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.0880}} \\
Time Since Launch & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0626}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0550}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.0804}} \\
Return (11th--15th) & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0300}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0445}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.1010}} \\
Return (1st) & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0377}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0573}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.0538}} \\
Return (all) & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0457}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0564}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.0310}} \\
Trader Purchase Quantity & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0240}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0393}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.0548}} \\
Time Since First Trade & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0446}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0259}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.0340}} \\
Number of Trades & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0157}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0426}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.0298}} \\
Trader Purchase Price & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0106}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0314}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.0398}} \\
Bump Bot & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0428}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0245}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.0051}} \\
Sniper Bot & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0280}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0364}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.0072}} \\
Bundle Bot & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0394}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0205}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.0059}} \\
Time Since Last Trade & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0162}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0289}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.0172}} \\
Comment Bot & \multicolumn{1}{|@{}l@{}|}{\databarLASSO{0.0110}} & \multicolumn{1}{|@{}l@{}|}{\databarNN{0.0123}} & \multicolumn{1}{|@{}l@{}|}{\databarXGB{0.0012}} \\
\bottomrule
\end{tabularx}

==> Tables/wallet.tex <==
\begin{tabular}{l|c|c|c}
\hline
           & \multicolumn{2}{c|}{\textbf{Predicted}} & \\
\cline{2-3}
\textbf{Actual} & TRUE & FALSE & \textbf{Total} \\
\hline
TRUE   & 4,773 & 238,169 & 242,942 \\
FALSE  & 2,106 & 369,282 & 371,388 \\
\hline
\textbf{Total} & 6,879 & 607,451 & 614,330 \\
\hline
\end{tabular}

